Unsupervised Methods for Identifying Pass Coverage Among Defensive Backs with NFL Player Tracking Data

Analysis of player tracking data for American football is in its infancy, since the National Football League (NFL) released its Next Gen Stats tracking data publicly for the first time in December 2018. While tracking datasets in other sports often contain detailed annotations of on-field events, annotations in the NFL's tracking data are limited. Methods for creating these annotations typically require extensive human labeling, which is difficult and expensive. We begin tackling this class of problems by creating annotations for pass coverage types by defensive backs using unsupervised learning techniques, which require no manual labeling or human oversight. We define a set of features from the NFL's tracking data that help distinguish between "zone" and "man" coverage. We use Gaussian mixture modeling and hierarchical clustering to create clusters corresponding to each group, and we assign the appropriate type of coverage to each cluster through qualitative analysis of the plays in each cluster. We find that the mixture model's "soft" cluster assignments allow for more flexibility when identifying coverage types. Our work makes possible several potential avenues of future NFL research, and we provide a basic exploration of these in this paper.

==> old.tex <==
Our two clustering approaches, HC and GMM, show some agreement in their cluster labels, but are not close to being in full agreement.  The four fold plot in Figure \ref{fig:fourfold} demonstrates this.

\begin{figure}[h]
  \centering
  \includegraphics[keepaspectratio, width=0.7\textwidth]{figures/4-fold.png}
  \caption{Four Fold Plot of the two clustering models used.}
  \label{fig:fourfold}
\end{figure}

Four fold plots provide a visualization of a 2-by-2 contingency table, and allow for a visual inspection of the independence or association between the two underlying dichotomous variables \citep{fourfold}.  This particular plot shows the association of the two-cluster solutions for GMM and HC.  We see GMM labels over 9000 coverages as ``man,'' and over 6000 coverages as ``zone,'' where a single coverages refers to a single DB's coverage type on a single play.  HC, on the other hand, yields a much more unbalanced clustering, with over 14,500 coverages labeled ``man,'' and only about 2000 coverages labeled zone.  Moreover, the plot provides visual representation of a chi-square test for independence of the two clusterings.  Specifically, since the 95\% confidence bands on adjacent folds do not overlap, we can reject the null hypothesis of independence.  This is to be expected, since we fit the two clusterings on the same data and using the same features, so their labels should be associated.

Another takeaway from this plot is that HC seems to struggle to identify zone coverage.  The GMM predicted zone 42\% of the time and man 58\% of the time. The HC model predicted zone 12\% of the time and man 88\% of the time. Furthermore, there were 5760 coverages where the highest cluster membership probability from GMM indicated zone coverage, but the hard cluster assignment from HC indicated man coverage.  While GMM is by no means ground truth, the class imbalance in the HC results is not favorable, leading us to conclude that the GMM model is a better fit.  The three plays detailed in the next section provide an illustration of the results of the clustering process, and help demonstrate why the GMM model is favorable in this context.
